Online Evolutionary Batch Size Orchestration for Scheduling Deep Learning Workloads in GPU Clusters

Efficient GPU resource scheduling is essential to maximize resource utilization and save training costs for the increasing amount of deep learning workloads in shared GPU clusters. Existing GPU schedulers largely rely on static policies to leverage the performance characteristics of deep learning jobs. However, they can hardly reach optimal efficiency due to the lack of elasticity. To address the problem, we propose ONES, an ONline Evolutionary Scheduler for elastic batch size orchestration. ONES automatically manages the elasticity of each job based on the training batch size, so as to maximize GPU utilization and improve scheduling efficiency. It determines the batch size for each job through an online evolutionary search that can continuously optimize the scheduling decisions. We evaluate the effectiveness of ONES with 64 GPUs on TACC's Longhorn supercomputers. The results show that ONES can outperform the prior deep learning schedulers with a significantly shorter average job completion time.

==> section/implementation.tex <==
\section{Implementation}
\label{sec:impl}

\subsection{Overview}

ONES consists of a central controller and managers that are distributed on each node.
The components communicate with each other by remote calls of the RPyC library \cite{rpyc}.

\textbf{Central controller:} the controller accepts job submissions and executes the scheduler to make scheduling decisions.
The information of each job is also stored at the controller.

\textbf{Distributed managers:} the managers execute workers on the GPU devices and are responsible for information exchange between workers and the controller.
The managers also continuously collect training performance as well as the cluster status information for the controller.

ONES can be deployed as an independent resource manager for GPU resources, or on the top of common cluster resource manager such as Kubernetes \cite{k8s} with GPU support.
The scheduler exposes an API for users to submit jobs with training scripts, initial batch sizes and corresponding learning rates.
Then it continuously optimizes the scheduling solution and deploys the optimal schedule on the GPUs in the shared cluster.
When deployed on the top of some cluster resource manager such as Kubernetes, the scheduler acts as an broker between users and the resource manager by determining resource allocation and then running each worker of the jobs on a specified GPU.


